Feature-Oriented Defect Prediction: Scenarios, Metrics, and Classifiers

Several software defect prediction techniques have been developed over the past decades. These techniques predict defects at the granularity of typical software assets, such as components and files. In this paper, we investigate feature-oriented defect prediction: predicting defects at the granularity of features -- domain-entities that represent software functionality and often cross-cut software assets. Feature-oriented defect prediction can be beneficial since: (i) some features might be more error-prone than others, (ii) characteristics of defective features might be useful to predict other error-prone features, and (iii) feature-specific code might be prone to faults arising from feature interactions. We explore the feasibility and solution space for feature-oriented defect prediction. Our study relies on 12 software projects from which we analyzed 13,685 bug-introducing and corrective commits, and systematically generated 62,868 training and test datasets to evaluate classifiers, metrics, and scenarios. The datasets were generated based on the 13,685 commits, 81 releases, and 24, 532 permutations of our 12 projects depending on the scenario addressed. We covered scenarios such as just-in-time (JIT) and cross-project defect prediction. Our results confirm the feasibility of feature-oriented defect prediction. We found the best performance (i.e., precision and robustness) when using the Random Forest classifier, with process and structure metrics. Surprisingly, single-project JIT and release-level predictions had median AUC-ROC values greater than 95% and 90% respectively, contrary to studies that assert poor performance due to insufficient training data. We also found that a model trained on release-level data from one of the twelve projects could predict defect-proneness of features in the other eleven projects with median AUC-ROC of 82%, without retraining.

==> Makefile <==
TEX=*.tex

BIB=*.bib

IMGS=imgs/*.pdf

main.pdf: $(TEX) $(BIB) $(IMGS)
	pdflatex main.tex &&\
	bibtex   main &&\
	pdflatex main && \
	pdflatex main

cr: main.pdf
	embedfonts main.pdf 

clean: 
	rm -f *~ *.aux *.bbl *.bbg *.log *.orig *.log *.pdf *.blg; find .. -type f -name '*~' -o -name '*.bak' -o -name 'Rplots.pdf' -o -name '*.backup' -o -name '*.orig' | xargs rm -f 
         
	


==> discussion.tex <==
\section{Perspectives and Directions}
Our results give rise to the following research directions.

\parhead{Compare file-based and feature-based defect prediction.} To understand the benefits of feature-oriented defect prediction, we shall compare the performance of classifiers on the same set of projects at the two granularity levels (file and feature), and the number of files predicted defective at each level. We shall also investigate whether any correlations exist between project characteristics (e.g., language, average feature size, frequency of changes, sizes of changes, etc.) and performance to investigate project-specific characteristics that may affect performance.

\parhead{Apply feature metrics to file-granularity defect prediction.} 
Even when just performing defect prediction at the granularity of files, we believe that taking information about features into account (with dedicated feature metrics) might improve prediction accuracy.
To study this conjecture, a feasible direction is to map our feature metrics back to relevant files, derive a metrics set with mixed file and feature information, and study the impact on prediction quality.
To this end, we plan to perform a further study, in which we compare this setup to traditional file-based feature prediction.


\parhead{Predict unwanted feature interactions}. Unwanted feature interactions\,\cite{apel2014feature} are a special kind of bug, which, when taken into account, may improve the predictive ability of defect prediction techniques, as well as provide meaningful insights regarding whether some machine learning classifiers perform better than others on specific kinds of bugs. While there is work on predicting feature interactions\,\cite{fischer2018predicting}, predicting \emph{unwanted} feature interactions has not been attempted yet, to the best of our knowledge.
To identify unwanted feature interaction bugs, one possible direction is to apply techniques for identifying variability-aware bugs, such as the one proposed by Abal et al.\,\cite{abal201442}. Another is to automatically generate test cases for features and use these as partial specifications of a feature behavior (similar to what has recently been done for semantic merge-conflict detection\,\cite{leuson2020testconflicts}), then exploit these test cases for revealing unwanted feature behavior when features interact.

%While our nesting depth metric allows to some extent to account for unwanted feature interactions, it is conceivable to use dedicated feature interaction detection techniques for supporting more advanced feature interactions.
 
\parhead{Change-based defect prediction for features.}  While our study has focused on release-based defect prediction, investigating the prediction of defective features whenever developers commit a new change would contribute to defect prediction techniques that provide immediate feedback to developers.

\parhead{Rich feature metrics.} We used feature metrics calculated upon code structure and project history. However, features carry more semantics and richer information, referred to as features facets (e.g., position in the hierarchy or architectural responsibility)\,\cite{berger.ea:2015:feature,krueger2018marlin,kruger2019my}. We conjecture crafting metrics taking such facets into account can improve prediction accuracy further.

\parhead{Improve generalizability.} Expanding our dataset to include more software projects, as well as considering other machine learning techniques, such as deep learning, can improve our classification results and the generalizability of our technique. Furthermore, investigating cross-project defect prediction is one other possible direction. Here, we hope to gain insights such as whether developers can reuse classification models for unseen projects or classifiers need to be retrained for such projects. 

==> evaluation.tex <==
\section{Evaluation}

In what follows, first, we present our evaluation metrics, second, we present our results and discuss their implications.


\subsection{Evaluation Metrics}
\label{subsec:metrics}
To compare the classifiers with regard to prediction quality, we consider two types of evaluation metrics, commonly used for this purpose in the field of information retrieval\,\cite{Sammut2017}.
First, \textit{precision}, \textit{recall}, and \textit{F-score}, which quantify information about the percentage of true and false predictions, based on an available \textsl{confusion matrix}.
Second, \textit{receiver operating characteristic} (ROC) curves and the associated \textit{area under curve} (AUC), which provide a visual and more robust way for assessing prediction quality than confusion-matrix-based metrics.

All our evaluation metrics assume a \textit{ground truth}, specifying for each given class the entries that belong to it (positives) and those that do not (negatives).
In our case, entries are features with regard to a given release.
The classes are \textit{defective} and \textit{clean}.
The ground truth was constructed in the labeling step during dataset construction (see Sect.~\ref{sec:dataset}).

\begin{table}[b]
\vspace{-.3cm}
\centering
\caption{Training times per metric set (in seconds)}
\vspace{-.3cm}
\label{tab:training-times}
\begin{tabular}{lrrr} 
\toprule
    & \metRod\ & \metA\ & \metB\ \\ 
\midrule
J48 & $0.44$    & $0.24$  & $0.46$               \\
KNN & $0.01$    & $0.02$  & $0.01$               \\
LR  & $0.29$    & $0.09$  & $0.14$               \\
NB  & $0.03$    & $0.03$  & $0.03$               \\
NN  & $51.85$   & $53.13$ & $65.34$              \\
RF  & $10.89$   & $6.04$  & $5.83$               \\
SVM & $0.6$     & $0.75$  & $1.65$               \\
\bottomrule
\end{tabular}
\end{table}


%Most of these metrics can be calculated using values from a so-called confusion matrix and all of them measure the performance of the predictions of classifiers from different points of view. In the case of a binary classification, as this work was based on, this matrix consists of four groups whose values indicate whether the respective classifier could correctly or incorrectly assign an object to one of the two target classes\,\cite{Sammut2017}. In connection with such matrices, the two target classes are called "positive" and "negative". For this work the positive class is assigned to the label "defective" and the negative class to the label "clean". The form of a general confusion matrix is shown in \autoref{fig:confu}.

%\begin{figure}[H]
    %\centering
    %\includegraphics[width=0.4\textwidth]{images/Confusion}
    %\caption{General confusion matrix\label{fig:confu}}
%\end{figure}

\parhead{Recall, Precision, and F-score.} 
We follow the standard definition of precision, recall, and F-score.
Intuitively, recall quantifies how exhaustively the classifier identified all entries of the class, comprised of true positives (TP) and false negatives (FN), respectively. 
Precision quantifies the percentage of true positives (TP) among all entries assigned to a particular class (also including false negatives, FN).
The F-score is the harmonic mean of precision and recall, representing a balance between both.
In contrast to other confusion-based-matrix (e.g., accuracy), these metrics are considered as useful on imbalanced datasets, such as ours.
These metrics are computed as follows:

\smallskip
%The WEKA tool used for training the classifiers has the option of outputting confusion matrices for the tests performed on the classifiers. Based on the values of the assignments to the groups mentioned above, the following evaluation metrics were calculated:
%\\
%\begin{itemize}
%\item $\text{Accuracy} = \frac{TP+TN}{TP+TN+FP+FN}$ \\
\noindent{}$\text{Recall} = \frac{TP}{TP+FN}$ \ \ \ $\text{Precision} = \frac{TP}{TP+FP}$ \ \  \ $\text{F-score} = \frac{2TP}{2TP+FP+FN}$ 
%\end{itemize}

\smallskip


\medskip
\noindent{}\textbf{ROC-AUC.} 
We determined the ROCs and AUCs of the individual classifiers. These have the benefit that they represent performance in a visual, understandable way, while at the same time making the quality assessment more robust:
Precision, recall, and F measure depend on a predefined threshold, which is used in the classifiers to assign each instance to a class.
A robust classifier shows good predictive ability regardless of the chosen threshold value.

ROC curves encode this intuition, by describing the relationship between the TP rate (a.k.a. recall, y axis) and the FP rate (x axis), indicating the proportion of predictions that are incorrectly evaluated as positive\,\cite{Sammut2017,Alpaydin2010}. 
The FP rate is calculated as follows:

\smallskip
\begin{center}
\noindent{}\text{FP rate} = $\frac{FP}{FP+TN}$
\end{center}

\medskip
Datapoints on the curve are obtained by taking into account all possible values for the threshold that determines when an instance is assigned to a particular class. 

The AUC area indicates the extent to which a classifier is able to make correct predictions under a changing threshold value. The higher this value is, the more robust the classifier is in making correct predictions.
The ideal value is 1.0, whereas a value of 0.5 indicates a predictive ability on the same level as random guessing.

\subsection{RQ1---Metrics and Classifiers: Results}
\looseness=-1

Using the classifiers we trained based on our dataset (see \autoref{sec:dataset}) and the three considered metric sets (see \autoref{sec:metrics}), we studied two research questions:

\begin{itemize}[leftmargin=*]
	\item \textbf{RQ1.1}: What is the effect of using different types of feature metrics (structural and process) on prediction quality?
	\item \textbf{RQ1.2}: Which particular feature metrics contribute most strongly to prediction quality? 
	\item \textbf{RQ1.3}: What is the effect of using different classifiers on prediction quality?
	%\item \textbf{RQ3}: What is the effect of our metric sets to prediction quality, compared to existing work?
\end{itemize}

Within RQ1, we implicitly compare our contribution to the most closely related work: our two new metric sets are compared to the one from \rodrigo\\,\cite{Queiroz2016}, who proposed the only other dedicated metric set for feature-oriented defect prediction.

\tabref{tab:eval-metrics} and \figref{fig:roc-feat} in combination give an overview of our results.
\tabref{tab:eval-metrics} provides all calculated precision, recall, F-score, and AUC values.
For each classifier and evaluation metric, the top value (best-perfoming metric set) is highlighted in bold.
\Figref{fig:roc-feat} shows ROCs for three representative classifiers (top performer, average performer, worst performer in terms of AUC) in combination with all three metrics sets.
For reference, AUC values of all cases are shown in the table.

\input{tables/evaluation}
\input{tables/rq2table}


%This chapter serves to evaluate the classifiers explained in the previous chapter, which are based on the data set presented above and which were built on the basis of data from 12 feature-based software projects. The data set consist of the attributes and the label as columns and in the rows the corresponding values for each feature aggregated by release. 
%The evaluation is done by different evaluation metrics and based on values of so-called confusion matrices and ROC curves.

%q\subsubsection*{Results and comparison of the feature-based classifiers}
%
%The presentation of the results starts with those of the classifiers of the feature-based data set. Based on the results of the evaluation metrics, performance can be measured and interpreted in terms of predicting faulty or error-free features. 

\parhead{RQ1: Effect of metric sets.} 
Based on precision, recall, and F-score, we generally observe a moderate tendency that classifiers performed best when using \metB, for which we observed weighted averages between 0.66--0.85, 0.70--0.85 and 0.68--0.83 respectively.
The corresponding ranges for the case of  \metA\ and \metRod\ are 0.58--0.84, 0.70--0.83 and 0.63--0.82,
and  0.55--0.84, 0.71--0.84 and 0.61--0.82, respectively.
The quality difference is particularly pronounced when considering the top values (printed in bold):
In all classifiers except for SVM, \metB\ shows the top value for precision, recall, and F-score.
Two noteworthy observations are the case of NB, where all evaluation metrics take the same values over all metrics sets, and SVM, where \metRod\ outperforms \metA\ and \metB.
Considering the two classes \textit{clean} and \textit{defective}, we generally find higher F-scores in the more advanced metric sets, and a better ability to predict clean than defective instances for all metric sets.


Considering ROCs and AUCs sheds light on the effect of the metric sets on robustness.
We generally find a clear tendency of \metB\ to highest robustness, i.e., more stability with regard to different values for the threshold used for assigning instances to classes (reflected by a steeper initial incline in the ROC curves).
In 5 out of 7 cases, the AUC for \metB\ shows a solid value between 0.74 and 0.82.
The AUC for \metB\ is consistently greater or equal to that of \metA\, in some cases strongly so, including the top performer NN (0.79 vs. 0.61).
The highest achieved value for \metRod\ is 0.64.
The SVM classifier is an exception to all other cases: for \metA\ and \metB\, we observe worse performance (0.49) than from random guessing (0.5); corresponding to a nearly-linear ROC.
%We explain this observation with a mismatch between the assumptions of SVM: 
%having a large sets of metrics makes it difficult to find a support vector.
A possible explanation for the preferable robustness of \metB\ in most classifiers is the availability of more diverse metrics, providing a richer information source for predictions.

\parhead{RQ2: Effect of individual metrics.} 
We determined the effect of individual metrics by applying an attribute selection method.
Such methods heuristically determine the effect of attributes, in our case metrics, with regard to a classifier's predictive ability.
We used a standard method provided by  Weka (\texttt{weka.attributeSelection. ClassifierAttributeEval} together with the \texttt{Ranker} class).
This method runs the considered classifier several times with different subsets of the entire metric set, and outputs an influence measure between 1.0 and -1.0 for each considered metric, quantifying the influence of the metric to the prediction result.
We applied the method to all 21 classifier instances (7 classifiers with 3 metric sets).

We present an overview of the results in \autoref{tab:eval-metrics}, showing the three top performers from RQ1 and the 
average over all 21 classifier instances.
The most influential metric for each classifier is highlighted in bold.
Generally, the obtained values are very similar for RF and J48, perhaps unsurprisingly, since RF and J48 are both based on the decision tree paradigm.
For NN, only three non-zero values are reported, which, however, agree with the reported values for the other two top classifiers.
We observe striking cases of large standard deviations, most pronounced in the case of FADDL, which has the most positive impact for the RF classifier (0.058), while, on average, leading to a strong negative influence (-0.03).
Despite the observation in RQ1 that the inclusion of structure metrics leads to improved results compared to only process metrics, the effect of each individual structure metric is moderate compared to the process metrics.
This indicates that structure metrics seem to play a non-negligible, but supplementary role for the observed results.


\parhead{RQ3: Effect of classifiers.} 
\looseness=-1
As a general observation, in most cases, the prediction quality of the same classifier varied strongly based on the considered metrics set (see RQ1).
It is, therefore, more meaningful to compare combinations of classifiers and metrics, rather than classifiers alone.
Considering weighted averages, we observe values for precision between 0.70--0.85, for recall between 0.62--0.85, and for F-measure between 0.61--0.83.
The best-performing classifiers with regard to F-measure were NN and RF, both in combination with \metB\ showing an F-measure of 0.83.
NN also shows the best average-weighted recall (0.85), while RF shows the top average-weighted precision (0.85).
With a value of 0.82 for \metB, J48 also achieved above-average performance.
%This was followed by the KNN classifier with $78\%$. With values of $66\%$ and $67\%$ respectively, the classifiers LR, NN, and SVM performed the worst. Thus, they determined a wrong result in more than $30\%$ of the predictions. What is striking about these results is the high performance of both decision tree-based classifiers J48 and RF. 

Considering individual classes, similar to the comparison between metrics, the results for the label \textit{defective} are generally worse than those of the label \textit{clean}.
The best precision for predicting clean files, 0.83, is observed for SVM in combination with \metRod.
However, this value is traded off for the worst observed recall for that label (0.12).
Note that the seemingly contra-intuitive average score of 0.78 for this combination results from averaging over the individual F-scores for class labels (0.21 and 0.91).

%The results of the further evaluation metrics TP rate / recall, FP rate, precision and F-score are divided according to the values of the target class, "defective" and "clean". In addition, the mean value of the results of both values of the target class is given. It displays the performance aggregated for both values and is ideally $1.00$ or $0.00$ for the FP rate.

%The best results in comparison were observed for by the RF classifier for the label "defective". $66\%$ of the actually defective data points were also predicted as such and only $12\%$ of the data points were falsely predicted as defective. The Precision and F-Score values are $53\%$ and $59\%$ respectively, at an average level. The J48 classifier achieved comparable results. SGD and SVM have the worst overall values. They actually detected defective data points with an accuracy of $34\%$ and $23\%$ respectively. The other classifiers operated at an average level. The respective mean values can be considered to compare the overall performance of the classifiers for both labels. Here again, the RF classifier performs best. The values for TP rate, precision and F-score are in the range of over $73\%$ and are thus comparatively above average. The FP rate of $23\%$, which is mainly due to the results regarding the label "clean", is at the lowest level of all classifiers. Again, the results of the decision tree based classifier J48 are at a similar level. The classifiers KNN and NB show average performance due to their high FP rate values. In total, the values of the classifiers LR, NN, SGD and SVM show that they have the worst performance in comparison. Especially the FP rates of over $43\%$ are at a high, undesirable level. 



%\paragraph{ROC curves und AUC areas}

%The interpretation of the ROC curves and ROC ranges is based on the presented scheme. The ROC curves are shown together with the values of the AUC ranges. The plots output by WEKA and unchanged are shown. The displayed colour gradients of the curves do not illustrate any information relevant for this purpose and can therefore be ignored.


Considering ROC curves and AUC areas, we again observe a large inter-classifier variability.
Still, the two top classifiers with regard to precision, recall, and F-balance also have the two highest observed AUC values:
RF with 0.82, and NN with 0.79, indicating that these classifiers a good robustness while ensuring high predictive ability. An interesting observation is that the minimal AUC value achieved per classifier was never higher than 0.61, close to random guessing. In contrast, in four out of seven cases, a maximal value of 0.78 could be observed -- illustrating again that the choice of metric set is a key decisive factor for the success or failure of a particular predictor.

\parhead{Summary.} 
We find a strong effect of metric selection on the classifier performance.
Remarkably, some classifiers become only feasible alternatives when used in combination with a suitable metric set.
In most cases, we notice that considering a greater selection of more diverse metrics (that we introduce in this paper) lead to improved performance, including the identified top performers NN and RF.
However, this tendency does not apply to all cases: a remarkable counterexample are SVMs, where the predictive ability declines with the availability of more metrics. Hence, identifying a metric set that improves the performance of the considered classifier appears to be a key prerequisite to successful adoption of machine learning techniques for feature-based defect prediction.

%It can be seen that no ROC curve approximates the ideal case presented. The best prediction performance is again shown by the RF Classifier with a AUC area of $0.84$. The NB Classifier shows a slightly lower performance with a ROC range of $0.80$. The classifiers J48 and KNN show an average performance of $0.77$ and $0.72$, respectively, with respect to the AUC area. The performance of the LR and NN classifiers are in the lower average. The SGD and SVM classifiers show the undesired case of a ROC curve bisecting the angle. This is also reflected in the AUC areas. The predictions thus approach a random guessing instead of being precise as desired.

%\paragraph{Summary}
%
%In each of the categories of metrics considered, the J48 and RF decision-tree-based classifiers proved to be the most performant compared to the other classifiers. The RF classifier usually also achieved a slightly higher performance. The algorithms underlying the classifiers seem to be best able to process the given feature-based data set with its eleven attributes with respect to the development of the derivation function for predicting new data.
%
%The classifiers SGD and SVM always showed the worst performance in comparison for each category of evaluation metrics. It was also found that the predictions of these classifiers approached random rates. Thus, the feature-based dataset does not seem to be suitable for these classification algorithms. Reasons for this could be a too small number of instances or a too high number of attributes.

%\subsubsection*{Results and comparison of the file-based classifiers}
%
%This section is used to evaluate and compare the classifiers of the file-based data sets. The reason for this comparison is to measure the influence of the feature-based metrics on the predictions of a classical file-based method taken from the scientific literature\,\cite{Moser2008}. The division of this section is similar to the previous section. By considering the results of the evaluation metrics of both data sets, the influence of the feature-based metrics in the extended file-based data set on the performance of the predictions can be analyzed. 
%
%\paragraph{Confusion matrices}
%
%The confusion matrices of the file-based datasets are listed in \autoref{tab:mat-eval}. The parent columns are arranged into the "simple" and the extended dataset. Both datasets contain the same number of records, so the "total" columns are identical. A brief analysis of the "defective" - "real defective" fields shows that only very few actually defective data points were actually predicted to be defective. This is also reflected in the further results of the evaluation metrics.
%
%\begin{table}[t]
%\centering
%\caption{Confusion matrices of the file-based data sets}
%\label{tab:mat-eval}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{llrrrrrr} 
%\hline
%                     &                & \multicolumn{3}{c}{„simple“ file-based data set} & \multicolumn{3}{c}{extended file-based data set}  \\ 
%\cline{3-8}
%\multicolumn{1}{c}{} & predicted ->    & defective & clean     & total                    & defective & clean     & total                     \\ 
%\hline
%\multirow{3}{*}{J48} & real defective & $11$      & $102$     & $113$                    & $10$      & $103$     & $113$                     \\
%                     & real clean     & $911$     & $20.923$  & $21.834$                 & $1.074$   & $20.760$  & $21.834$                  \\
%                     & total          & $922$     & $21.025$  & $21.947$                 & $1.084$   & $20.863$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{KNN} & real defective & $29$      & $84$      & $113$                    & $23$      & $90$      & $113$                     \\
%                     & real clean     & $5.209$   & $16.625$  & $21.834$                 & $5.092$   & $16.742$  & $21.834$                  \\
%                     & total          & $5.238$   & $16.709$  & $21.947$                 & $5.115$   & $16.832$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{LR}  & real defective & $36$      & $77$      & $113$                    & $32$      & $81$      & $113$                     \\
%                     & real clean     & $2.520$   & $19.314$  & $21.834$                 & $2.689$   & $19.145$  & $21.834$                  \\
%                     & total          & $2.556$   & $19.391$  & $21.947$                 & $2.721$   & $19.226$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{NB}  & real defective & $77$      & $36$      & $113$                    & $82$      & $31$      & $113$                     \\
%                     & real clean     & $18.700$  & $3.134$   & $21.834$                 & $18.755$  & $3.079$   & $21.834$                  \\
%                     & total          & $18.777$  & $3.170$   & $21.947$                 & $18.837$  & $3.110$   & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{NN}  & real defective & $6$       & $107$     & $113$                    & $6$       & $107$     & $113$                     \\
%                     & real clean     & $4.341$   & $17.493$  & $21.834$                 & $697$     & $21.137$  & $21.834$                  \\
%                     & total          & $4.347$   & $17.600$  & $21.947$                 & $703$     & $21.244$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{RF}  & real defective & $7$       & $106$     & $113$                    & $4$       & $109$     & $113$                     \\
%                     & real clean     & $382$     & $21.452$  & $21.834$                 & $363$     & $21.471$  & $21.834$                  \\
%                     & total          & $389$     & $21.558$  & $21.947$                 & $367$     & $21.580$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{SGD} & real defective & $22$      & $91$      & $113$                    & $20$      & $93$      & $113$                     \\
%                     & real clean     & $1.260$   & $20.574$  & $21.834$                 & $1.203$   & $20.631$  & $21.834$                  \\
%                     & total          & $1.282$   & $20.665$  & $21.947$                 & $1.223$   & $20.724$  & $21.947$                  \\ 
%\hline
%\multirow{3}{*}{SVM} & real defective & $22$      & $91$      & $113$                    & $21$      & $92$      & $113$                     \\
%                     & real clean     & $1.041$   & $20.793$  & $21.834$                 & $1.024$   & $20.810$  & $21.834$                  \\
%                     & total          & $1.063$   & $20.884$  & $21.947$                 & $1.045$   & $20.902$  & $21.947$                  \\
%\hline
%\end{tabular}
%}
%\end{table}
%
%\paragraph{Accuracy, TP rate / recall, FP rate, precision, F-score}
%
%The results of these metrics are presented in \autoref{tab:met-results}. The parent columns are again represented by the two data sets.
%
%\begin{table}[t]
%\centering
%\caption{Results of the evaluation metrics of the file-based data sets}
%\label{tab:met-results}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{llrrrrrr} 
%\toprule
%                     &              & \multicolumn{3}{c}{"simple" file-based data set} & \multicolumn{3}{c}{extended file-based data set}  \\ 
%\cline{3-8}
%                     &              & defective & clean           & mean               & defective & clean           & mean                \\ 
%\midrule
%\multirow{5}{*}{J48} & accuracy     & \multicolumn{2}{r}{result:} & $0,95$             & \multicolumn{2}{r}{result:} & $0,95$              \\
%                     & TPR / recall & $0,10$    & $0,96$          & $0,53$             & $0,09$    & $0,95$          & $0,52$              \\
%                     & FP rate      & $0,04$    & $0,90$          & $0,47$             & $0,05$    & $0,91$          & $0,48$              \\
%                     & precision    & $0,01$    & $1,00$          & $0,51$             & $0,01$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,02$    & $0,98$          & $0,50$             & $0,02$    & $0,97$          & $0,50$              \\ 
%\midrule
%\multirow{5}{*}{KNN} & accuracy     & \multicolumn{2}{r}{result:} & $0,76$             & \multicolumn{2}{r}{result:} & $0,76$              \\
%                     & TPR / recall & $0,26$    & $0,76$          & $0,51$             & $0,20$    & $0,77$          & $0,49$              \\
%                     & FP rate      & $0,24$    & $0,74$          & $0,49$             & $0,23$    & $0,80$          & $0,52$              \\
%                     & precision    & $0,01$    & $1,00$          & $0,51$             & $0,00$    & $1,00$          & $0,50$              \\
%                     & F-score      & $0,01$    & $0,86$          & $0,44$             & $0,01$    & $0,87$          & $0,44$              \\ 
%\midrule
%\multirow{5}{*}{LR}  & accuracy     & \multicolumn{2}{r}{result:} & $0,88$             & \multicolumn{2}{r}{result:} & $0,87$              \\
%                     & TPR / recall & $0,32$    & $0,89$          & $0,61$             & $0,28$    & $0,88$          & $0,58$              \\
%                     & FP rate      & $0,12$    & $0,68$          & $0,40$             & $0,12$    & $0,72$          & $0,42$              \\
%                     & precision    & $0,01$    & $1,00$          & $0,51$             & $0,01$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,03$    & $0,94$          & $0,49$             & $0,02$    & $0,93$          & $0,48$              \\ 
%\midrule
%\multirow{5}{*}{NB}  & accuracy     & \multicolumn{2}{r}{result:} & $0,15$             & \multicolumn{2}{r}{result:} & $0,14$              \\
%                     & TPR / recall & $0,68$    & $0,14$          & $0,41$             & $0,73$    & $0,14$          & $0,44$              \\
%                     & FP rate      & $0,86$    & $0,32$          & $0,59$             & $0,86$    & $0,27$          & $0,57$              \\
%                     & precision    & $0,00$    & $0,99$          & $0,50$             & $0,00$    & $0,99$          & $0,50$              \\
%                     & F-score      & $0,01$    & $0,25$          & $0,13$             & $0,01$    & $0,25$          & $0,13$              \\ 
%\midrule
%\multirow{5}{*}{NN}  & accuracy     & \multicolumn{2}{r}{result:} & $0,80$             & \multicolumn{2}{r}{result:} & $0,96$              \\
%                     & TPR / recall & $0,05$    & $0,80$          & $0,43$             & $0,05$    & $0,97$          & $0,51$              \\
%                     & FP rate      & $0,20$    & $0,95$          & $0,58$             & $0,03$    & $0,95$          & $0,49$              \\
%                     & precision    & $0,00$    & $0,99$          & $0,50$             & $0,01$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,00$    & $0,89$          & $0,45$             & $0,02$    & $0,98$          & $0,50$              \\ 
%\midrule
%\multirow{5}{*}{RF}  & accuracy     & \multicolumn{2}{r}{result:} & $0,98$             & \multicolumn{2}{r}{result:} & $0,98$              \\
%                     & TPR / recall & $0,06$    & $0,98$          & $0,52$             & $0,04$    & $0,98$          & $0,51$              \\
%                     & FP rate      & $0,02$    & $0,94$          & $0,48$             & $0,02$    & $0,97$          & $0,50$              \\
%                     & precision    & $0,02$    & $1,00$          & $0,51$             & $0,01$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,03$    & $0,90$          & $0,47$             & $0,02$    & $0,99$          & $0,51$              \\ 
%\midrule
%\multirow{5}{*}{SGD} & accuracy     & \multicolumn{2}{r}{result:} & $0,94$             & \multicolumn{2}{r}{result:} & $0,94$              \\
%                     & TPR / recall & $0,20$    & $0,94$          & $0,57$             & $0,18$    & $0,95$          & $0,57$              \\
%                     & FP rate      & $0,06$    & $0,81$          & $0,44$             & $0,06$    & $0,82$          & $0,44$              \\
%                     & precision    & $0,02$    & $1,00$          & $0,51$             & $0,02$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,03$    & $0,97$          & $0,50$             & $0,03$    & $0,94$          & $0,49$              \\ 
%\midrule
%\multirow{5}{*}{SVM} & accuracy     & \multicolumn{2}{r}{result:} & $0,95$             & \multicolumn{2}{r}{result:} & $0,95$              \\
%                     & TPR / recall & $0,20$    & $0,95$          & $0,58$             & $0,19$    & $0,95$          & $0,57$              \\
%                     & FP rate      & $0,05$    & $0,81$          & $0,43$             & $0,05$    & $0,81$          & $0,43$              \\
%                     & precision    & $0,02$    & $1,00$          & $0,51$             & $0,02$    & $1,00$          & $0,51$              \\
%                     & F-score      & $0,04$    & $0,97$          & $0,51$             & $0,04$    & $0,97$          & $0,51$              \\
%\bottomrule
%\end{tabular}
%}
%\end{table}
%
%The comparison between the accuracies of the data sets shows that the integration of feature-based metrics has no significant impact on the performance of the predictions for six out of eight classifiers. The achieved values of the Accuracies are on the same level there. The NB classifier achieves the worst accuracy in comparison with the other classifiers with about $15\%$ accuracy. It seems to be unable to process the high number of data sets correctly. The classifiers KNN and LR achieved above average results with about $76\%$ and $87\%$ respectively. With values of more than $90\%$, the classifiers J48, RF, SGD and SVM have extremely high values, whose validity should be questioned first. A consideration of the other evaluation metrics should be made.
%
%The NN classifier shows a conspicuous behaviour. There is a clear jump in values of about $18\%$ between the "simple" and the extended data set. This anomaly should also be analyzed and interpreted using the other evaluation metrics. It may indicate that the classifier of the extended dataset can make more accurate predictions by adding the additional attributes, or that the predictions are negatively affected by the addition of the additional attributes, thus distorting the results.
%
%The results of the further evaluation metrics of both data sets again show the trend that only a few defective data points were actually predicted as defective. With TP rates of $68\%$ and $74\%$ respectively, the NL classifiers achieved the highest hit rates. The other classifiers are significantly lower with values of $32\%$ at most. The other metrics of the "defective" columns also represent extremely weak results. Noticeable are the very high FP rates of the NB classifiers, which clearly weaken the good results of the TP rates.
%
%The values of the "error-free" columns show very good values. Only the respective FP rates with over $68\%$ are clearly too high and show that the classifiers incorrectly predict many data points as "clean". An exception to this is again the NB classifiers, which achieved good values in terms of FP rates and precision, but have shortcomings in terms of TP rates and consequently the F-score. Furthermore, the different accuracies of the NN classifiers can be justified with the results of the other evaluation metrics. It can be seen that between the data sets the values of the TP rates and FP rates differ for both labels. Consequently, the F-scores also differ. These differences in the values lead to the different values of the Accuracies.
%
%The mean values show that the overall results are strongly influenced downwards by the values of the "defective" columns. They show that all classifiers make predictions at an average to below average level.
%
%\paragraph{ROC curves und AUC areas}
%
%The ROC curves and their associated AUC areas of the file-based datasets can be seen in \autoref{roc-file}. Again, the displayed color gradients of the curves do not convey any information relevant for this purpose and can therefore be ignored.
%
%A first look at the ROC curves of the classifiers shows a relatively uniform picture of curves that are very much oriented on the bisector and are uniform between the data sets. With the exception of the RF classifiers of both data sets, the curves with their associated ROC areas show a below-average to undesired performance (random rate of labels). With an ROC area of $0.71$, the RF classifiers have above average performance in the higher-level comparison.
%
%The comparison between the NN classifiers shows that the classifier of the simple dataset shows the undesired behaviour and at the same time makes inverse predictions. This means that in some cases it predicts the label "defective" instead of "clean" and vice versa. The curve as well as the ROC area of the classifier of the extended dataset, however, only show the undesired behavior in the form of random guessing of the predictions. This shows that the high accuracies of the NN classifiers shown in \autoref{tab:met-results} are probably caused by chance. In a further application of the test data, the results could have been different.
%
%\begin{figure*}[t]
%  \centering
%  \subfloat[][J48 "simple"\\AUC = $0,61$]{\includegraphics[width=0.25\linewidth]{images/j48_eval}} 
%  \subfloat[][J48 extended\\AUC = $0,61$]{\includegraphics[width=0.25\linewidth]{images/j48_eval_feat}}
%  \subfloat[][NN "simple"\\AUC = $0,37$]{\includegraphics[width=0.25\linewidth]{images/nn_eval}}
%  \subfloat[][NN extended\\AUC = $0,40$]{\includegraphics[width=0.25\linewidth]{images/nn_eval_feat}}
%  \qquad
%  \subfloat[][KNN "simple"\\AUC = $0,55$]{\includegraphics[width=0.25\linewidth]{images/knn_eval}}
%  \subfloat[][KNN extended\\AUC = $0,52$]{\includegraphics[width=0.25\linewidth]{images/knn_eval_feat}}
%  \subfloat[][RF "simple"\\AUC = $0,71$]{\includegraphics[width=0.25\linewidth]{images/rf_eval}} 
%  \subfloat[][RF extended\\AUC = $0,72$]{\includegraphics[width=0.25\linewidth]{images/rf_eval_feat}} 
%  \qquad
%  \subfloat[][LR "simple"\\AUC = $0,65$]{\includegraphics[width=0.25\linewidth]{images/lr_eval}}
%  \subfloat[][LR extended\\AUC = $0,61$]{\includegraphics[width=0.25\linewidth]{images/lr_eval_feat}}
%  \subfloat[][SGD "simple"\\AUC = $0,57$]{\includegraphics[width=0.25\linewidth]{images/sgd_eval}}
%  \subfloat[][SGD extended\\AUC = $0,56$]{\includegraphics[width=0.25\linewidth]{images/sgd_eval_feat}}
%  \qquad
%  \subfloat[][NB "simple"\\AUC = $0,48$]{\includegraphics[width=0.25\linewidth]{images/nb_eval}}
%  \subfloat[][NB extended\\AUC = $0,42$]{\includegraphics[width=0.25\linewidth]{images/nb_eval_feat}}
%  \subfloat[][SVM "simple"\\AUC = $0,57$]{\includegraphics[width=0.25\linewidth]{images/svm_eval}}
%  \subfloat[][SVM extended\\AUC = $0,57$]{\includegraphics[width=0.25\linewidth]{images/svm_eval_feat}}
%  \caption{ROC curves of the file-based data sets \label{roc-file}}
%\end{figure*}
%
%\paragraph{Summary}
%
%The results of all metrics showed an undifferentiated and unclear picture of the classifier performance for both data sets. The reason for the shown results is the unbalanced nature of the respective test data sets with only $1\%$ of "defective" instances. In order to get good results for this label, many correct predictions have to be made by the classifiers. However, this was not the case for the existing test dataset, so that many predictions were incorrectly assigned to the dominant label "clean", which then, however, show high FP rates as a result. This is also reflected in the mean values in \autoref{tab:met-results}. Due to the significantly weaker values of the "defective" columns, the total values represented by the mean value are influenced downwards. However, as explained earlier, it is not intended to compensate for the unbalanced nature of the test data sets using the SMOTE algorithm.
\input{rq2_featuremetricsOnFilePrediction}
\subsection{Threats to Validity}

\parhead{External validity.} 
To mitigate overfitting of our models, a key threat in machine learning, we used the typical separation of the dataset into test data and training data\,\cite{domingos2012few}.
Another standard technique to mitigate overfitting, cross validation, is not applicable to scenario, since it leads to the problematic situation of "using the future to predict the past", which is unrealistic for practical applications\,\cite{jimenez2019importance}.
While providing improved techniques for avoiding overfitting in defect prediction contexts is an open research issue, we observe good predictive ability for 12 systems of diverse context and size, which gives us some confidence that our models are not severely affected by overfitting.

Despite diversity and size of the projects in our dataset, studying a broader selection of software projects is desirable, as it would increase the generalizability of our findings.
We intend to aggregate larger datasets in future work, which would also contribute to our ongoing community initiative towards more mature benchmarks for techniques in the context of evolving variant-rich systems\,\cite{SMK19}.

\parhead{Internal validity.} 
As observed in \secref{sec:dataset}, we observed that some of our automatically retrieved features were not meaningful, as they  represented "header features", in the style of a certain C pattern.
While we manually processed all identified features to remove header features, it is possible that in some projects header features are not explicitly identified by names.
A possible solution could be enabled by a tool that automatically analyses the code to detect header features. Such a tool does not exist at the moment.
Still, the manual removal of the recognizable header features allowed us to  reduce the amount of these noise datapoints. Furthermore, we take a conservative approach by considering only features referenced through \hashifdef and \ifndef. We also do not explicitly exclude standard predefined macros such as \texttt{\small{\_\_FILE\_\_}}, \texttt{\small{\_\_LINE\_\_}}, etc., since we treat them as features with associated code if they are referenced through our selected preprocessor macros above.

\looseness=-1
During dataset creation, we rely on a mapping from all features changed in a particular release to the associated files.
This mapping is obtained from analyzing all commit change sets within the release.
Thus, a feature is considered relevant if it is mentioned in a diff (either within a changed line or in the context provided with change lines, which, per default, extends to three lines before and after changed lines).
This heuristic is subject to imprecision related to preprocessor macros outside the  provided context.
Extending the implementation to take into account all files 
is subject to future work.

%\subsubsection*{Heuristic for identifying corrective Commits}
%The heuristic for detecting corrective commits was changed during the course of the work. First, the entire commit message was analyzed for the presence of the keywords. However, this resulted in some commits being incorrectly identified as corrective. The reason for this was that the commit messages in some of the software projects used were very large in word count. These messages mentioned all the changes made by the commits, without exception. However, most of these changes were irrelevant for this purpose. It was found that the main statement or reason for the commit was in the first line of the commit message. The heuristics were then adjusted accordingly. A sample of corrective commits before and after the heuristic adjustment showed that the change caused irrelevant corrective commits to be removed.

\parhead{Construct validity.} 
Our ground truth for the identification of defective and clean features relies on an available heuristic technique, the SZZ algorithm. 
An associated threat is concerned with possible imprecisions of this algorithm.
According to a recent study\,\cite{Wen2019},  available implementations of SZZ, including those of PyDriller, can identify only about 69\% of all bug-introducing commits. In addition, about 64\% of the identified commits were found to be incorrectly identified.
These imprecisions arise from violations to implicit assumptions of the SZZ algorithm.
Furthermore, the authors of the study empirically found that the results of eight out of ten earlier studies were significantly influenced by the imprecise algorithm\,\cite{Wen2019}. This may, therefore, also apply to this work. However, there is currently no alternative method for identifying bug-introducing commits. Whenever an improved method becomes available, we will repeat the main steps of this work, taking the new method into account, and compare with our results.
